Highly-Efficient Persistent FIFO Queues

In this paper, we study the question whether techniques employed, in a conventional system, by state-of-the-art concurrent algorithms to avoid contended hot spots are still efficient for recoverable computing in settings with Non-Volatile Memory (NVM). We focus on concurrent FIFO queues that have two end-points, head and tail, which are highly contended. We present a persistent FIFO queue implementation that performs a pair of persistence instructions per operation (enqueue or dequeue). The algorithm achieves to perform these instructions on variables of low contention by employing Fetch&Increment and using the state-of-the-art queue implementation by Afek and Morrison (PPoPP'13). These result in performance that is up to 2x faster than state-of-the-art persistent FIFO queue implementations.

==> discussion.tex <==
\section{Discussion}
In order to evaluate \PLCRQ, we compare its performance with 
the state-of-the-art \PBComb\ and \PWFComb\ universal construction algorithms \cite{?} as 
implemented with 
``The Synch Framework'' \cite{?}. More specifically, we compare our implementation with the queue
implementation of these universal constructions \PBQueue\ and \PWFQueue. In \cite{?} there is an
extensive evaluation of \PBQueue\ and \PWFQueue, which shows that they outperform all the competitor
recoverable queue implementations. Specifically, \PBQueue\ is 2x faster than the next best competitor.
For our performance evaluation we used a machine equipped with NVDIMMs\footnote{The full 
specifications are
shown in Appendix~\ref{sec:evaluation}}, which shows that \PLCRQ\ can be up to 2x 
faster than \PBQueue. Due to space limitations, the evaluation section is presented in 
Appendix~\ref{sec:evaluation}.

==> main_algo/SW-code.tex <==
\begin{algorithm}[t]
\scriptsize
\caption{\PCRQ. Instances of $\Q$, \Head, and \Tail\ refer to $crq.\Q$, $crq.\Head$ and $crq.\Tail$.
This is the optimized algorithm that uses single writer objects to escape costly \pwbi\ operations 
on contended shared variable \Head. 
% Ignore code in blue to get the psuedocode for \CRQ.%
} \label{alg:pcrqsw}
\begin{multicols}{2}
\begin{algorithmic}[1]
\Function{Enqueue}{\crqV, $\itemX$}
    \State $\var{closedFlag}:$ integer, initially 0
    \While{\True{}} \label{pcrqsw:eqloop}
        \State $( \var{cb}, \localTail) \gets \Call{Fetch\&Increment}{\Tail}$ \label{pcrqsw:eqfaa}
        \If{$\var{cb} == 1$}    \Comment{closed bit is set}
            \If{\recoverycode{$\var{closedFlag} == 0$}} 
                \State \recoverycode{\pwb{\Tail}; \psync{}} \label{pcrqsw:closed-pwb-1}
                \State \recoverycode{$\var{closedFlag} \gets 1$}
            \EndIf
            \State \Return \CLOSED{} \label{pcrqsw:eqclosed-1}
        \EndIf
        \State $e\gets \Q[\localTail\bmod R]$ \label{pcrqsw:eqr1} \Comment{get item}
        \State $v\gets e.\var{val}$ \label{pcrqsw:eqr2} \Comment{get item's value}
        \State $( s,i) \gets ( e.s,e.\var{idx}) $ \label{pcrqsw:eqr3} \Comment{get safe bit and
            index}
        \If{$v == \bot$} \label{pcrqsw:eqbotchk}
            \If{$i\leq \localTail$ \textbf{and} ($s == 1$ \textbf{or} $\Head \leq \localTail$) \textbf{and} \\
                \hspace*{0.2cm} \Call{CAS2}{$\Q[\localTail\bmod R],( s,i,\bot) ,( 1,\localTail{},\itemX{}) $}} \label{pcrqsw:eqcas}
                \State \recoverycode{\pwb{$\Q[\localTail\bmod R]$};} \recoverycode{\psync{}} \label{pcrqsw:eqpwb}
                \State \Return \OK{} \label{pcrqsw:eqretOK}
            \EndIf
        \EndIf
        \State $\localHead{}\gets \Head{}$ \Comment{read \Head{}} \label{pcrqsw:headread}
        \If{$\localTail{}-\localHead{}\geq R$ \textbf{or} \Call{starving}{}}\label{pcrqsw:eqclosedchk}
            \State \Call{Test\&Set}{$\Tail{}.\var{cb}$} \label{pcrqsw:eqts}
            \State \recoverycode{\pwb{\Tail};} \recoverycode{\psync{}} \label{pcrqsw:closed-pwb-2}
            \State \recoverycode{$\var{closedFlag} \gets 1$}
            \State \Return \CLOSED{} \label{pcrqsw:eqclosedret}
        \EndIf
    \EndWhile
\EndFunction
\medskip% \Statex
%
%%% DEQUEUE FUNCTION %%%
\Function{Dequeue}{\crqV}
    \While{\True{}} \label{pcrqsw:dqouterloop}
        \State $\Head_i\gets \Call{Fetch\&Increment}{\Head}$ \label{pcrqsw:dqfaa}
        \State $\localHead \gets \Head_i$
        \State $e\gets \Q[\localHead\bmod R]$ \label{pcrqsw:dqr1} \Comment{read item}
        \While{\True{}}
            \State $v\gets e.v$ \label{pcrqsw:dqr2} \Comment{read item's value}
            \State $( s,i) \gets ( e.s,e.\var{idx})$ \label{pcrqsw:dqr3} 
            \If{$i>\localHead{}$} \label{pcrqsw:dqichk}
                \textbf{goto} line \ref{pcrqsw:fix} \label{pcrqsw:enddqr2}
            \EndIf
            \If{$v\neq \bot$} \label{pcrqsw:dqemptychk}
                \If{$i == \localHead{}$} \label{pcrqsw:dqhchk}
                    \If{\Call{CAS2}{$\Q[\localHead\bmod R]$,$( s,\localHead,v)$,$( s,
                    \localHead{}+R,\bot)$}} \Comment{dequeue transition} \label{pcrqsw:dqtran}
                        \State \recoverycode{\pwb{$\Head_i$};} \recoverycode{\psync{}} \label{pcrqsw:dqpwbHead}
                        \State \Return $v$ \label{pcrqsw:dqret}
                    \EndIf
                \Else
                    \If{\Call{CAS2}{$\Q[\localHead\bmod R],( s,i,v) ,( 0,i,v)$}} 
                    \label{pcrqsw:unsafe} \Comment{unsafe transition}
                        \State \textbf{goto} line \ref{pcrqsw:fix} \label{pcrqsw:endunsafe}
                    \EndIf
                \EndIf
            \Else
                \If{\Call{CAS2}{$\Q[\localHead\bmod R],( s,i,\bot) ,( s,\localHead+R,
                \bot)$}} \Comment{empty transition} \label{pcrqsw:empty-1}
                    \State \textbf{goto} line \ref{pcrqsw:fix} \label{pcrqsw:endempty}
                \EndIf
            \EndIf
        \EndWhile
        \State $( \var{cb},\localTail{}) \gets$ \Tail \label{pcrqsw:fix}
        \If{$\localTail{}\leq \localHead{}+1$} \label{pcrqsw:empty}
            \State \recoverycode{\pwb{$\Head_i$};} \recoverycode{\psync{}} \label{pcrqsw:dqpwbHead2}
            \State \Call{FixState}{\crqV}
            \State \Return \EMPTY \label{pcrqsw:endfix}
        \EndIf
    \EndWhile
\EndFunction
\medskip
%
%%% FIX STATE %%%
\Function{FixState}{crq}
\While{True}
    \State $h\gets$ \Call{Fetch\&Add}{crq.head, 0}
    \State $t\gets$ \Call{Fetch\&Add}{crq.tail, 0}
    \If{$\text{crq.tail}\neq t$}
        \State \textbf{continue}
    \EndIf
    \If{$h\leq t$}
        \State \Return
    \EndIf
    \If{$\Call{CAS}{\text{crq.tail}, t, h}$}
        \State \Return
    \EndIf
\EndWhile
\EndFunction
\medskip
%\end{algorithmic}
%\end{multicols}
%\begin{multicols}{2}
%\begin{algorithmic}[1]
%\setcounter{ALG@line}{58}
%
%%% RECOVERY FUNCTION %%%
\recoverycode{
\Function{Recovery}{}
%\LComment{Parameters}
\State $R\colon$ size of circular array
%\Statex
%\LComment{Implementation}
\State $\Head \gets \max_{i=1\ldots n} \Head_i$
\State $( \var{cb}, \localTail) \gets \Tail$ \label{pcrqsw:rec-tail-read}
\State $\Tail\gets ( \var{cb}, 0 )$
\For{$i\gets 0;\ i < R;\ i\texttt{++}$} \label{pcrqsw:rec-tail-loop}
    \If{$\Q[i].\var{val} \neq \bot$
	    \textbf{and} $\Tail < \Q[i].\var{idx} + 1$} \label{pcrqsw:rec-tail-occupiedchk}
	%        \LComment{occupied node and index is greater than current \Tail, hence update}
	        \State $\Tail\gets \Q[i].\var{idx} + 1$ \label{pcrqsw:rec-tail-set2}
    \ElsIf{$\Q[i].\var{val} == \bot$
    \textbf{and} $\Q[i].\var{idx} \geq R$} \label{pcrqsw:rec-tail-emptychk}
        \If{$\Tail < \Q[i].\var{idx} - R + 1$}
%            \LComment{empty node due to either a normal dequeue or an empty transition, and 
%            index $-R$ greater than current \Tail, hence update}
            \State $\Tail\gets \Q[i].\var{idx} - R + 1$ \label{pcrqsw:rec-tail-set1}
        \EndIf
    \EndIf
\EndFor
\If{$\Head>\Tail$} $\Tail\gets \Head$ \Comment{Empty queue} \label{pcrqsw:recemptycheck}
\Else \Comment{$\Head\leq \Tail$}
%    \LComment{Fix \Head\ to start from maximum index of unoccupied nodes $+1$}
    \State $\var{max} \gets \Head$ \label{pcrqsw:recinimax}
    \For{$i\gets \Head$;\ $i \bmod R \neq \Tail \bmod R$;\ $i\texttt{++}$} \label{pcrqsw:recmaxfor}
        \If{$\Q[i \bmod R].\var{val} == \bot$ \textbf{and}\\
        \hspace*{0.5em} $\Q[i \bmod R].\var{idx} - R > \var{max}$}
        \label{pcrqsw:recgtmax}
            \State $\var{max}\gets \Q[i \bmod R].\var{idx} - R + 1$
            \label{pcrqsw:recsetmax}
        \EndIf
    \EndFor
    \State $\Head \gets \var{max}$ \label{pcrqsw:rec-max-found}
%    \LComment{Fix \Head\ to start from minimum index of occupied nodes in $(\Head,\Tail]$}
    \State $\var{min} \gets \Tail$ \label{pcrqsw:rec-min-ini}
    \For{$i\gets \Head$;\ $i \bmod R \neq \Tail \bmod R$;\ $i\texttt{++}$}
        \If{$\Q[i \bmod R].\var{val} \neq \bot$
        \textbf{and} $\Q[i \bmod R].\var{idx} < \var{min}$
        \textbf{and} $\Q[i \bmod R].\var{idx} \geq \Head{}$} 
        \label{pcrqsw:recgteHead}
            \State $\var{min}\gets \Q[i \bmod R].\var{idx}$
        \EndIf
    \EndFor
    \If{$\var{min} < \Tail$} $\Head \gets \var{min}$ \label{pcrqsw:rec-min-found} \EndIf
\EndIf
%\LComment{Reset the rest of the array's positions}
\For{$i = \Head - 1;\ i \bmod R \neq \Tail \bmod R;\ i\texttt{--}$} \label{pcrqsw:resetloop}
    \State $\Q[i \bmod R] \gets ( 1, i+R, \bot)$ \label{pcrqsw:resetnodes}
\EndFor
%\LComment{Reset all safe flags to $1$}
\For{$i = 0;\ i < R;\ i\gets i + 1$} $\Q[i].s \gets 1$ \label{pcrqsw:resetsfloop1} \EndFor
\EndFunction        
}
\end{algorithmic}
\end{multicols}
\end{algorithm}


==> main_algo/per_crq_code.tex <==
\begin{algorithm}[t]
\scriptsize
\caption{\PCRQ, code for thread $p_i$. 
Ignore code in blue to get the pseudocode for \CRQ. 
Instances of $\Q$, \Head, and \Tail\ refer to $crq.\Q$, $crq.\Head$ and $crq.\Tail$. 
} \label{alg:pcrq}
\begin{multicols}{2}
\begin{algorithmic}[1]
\Function{Enqueue}{\crqV, $\itemX$}
    \State $\var{closedFlag}:$ integer, initially 0
    \While{\True{}} \label{pcrq:eqloop}
        \State $( \var{cb}, \localTail) \gets \Call{Fetch\&Increment}{\Tail}$ \label{pcrq:eqfaa}
        \If{$\var{cb} == 1$}    \Comment{closed bit is set}
            \If{\recoverycode{$\var{closedFlag} == 0$}} 
                \State \recoverycode{\pwb{\Tail}; \psync{}} \label{pcrq:closed-pwb-1}
                \State \recoverycode{$\var{closedFlag} \gets 1$}
            \EndIf
            \State \Return \CLOSED{} \label{pcrq:eqclosed-1}
        \EndIf
        \State $e\gets \Q[\localTail\bmod R]$ \label{pcrq:eqr1} \Comment{get item}
        \State $v\gets e.\var{val}$ \label{pcrq:eqr2} \Comment{get item's value}
        \State $( s,i) \gets ( e.s,e.\var{idx}) $ \label{pcrq:eqr3} \Comment{get safe bit and
            index}
        \If{$v == \bot$} \label{pcrq:eqbotchk}
            \If{$i\leq \localTail$ \textbf{and} ($s == 1$ \textbf{or} $\Head \leq \localTail$) \textbf{and} \\
                \hspace*{0.2cm} \Call{CAS2}{$\Q[\localTail\bmod R],( s,i,\bot) ,( 1,\localTail{},\itemX{}) $}} \label{pcrq:eqcas}
                \State \recoverycode{\pwb{$\Q[\localTail\bmod R]$};} \recoverycode{\psync{}} \label{pcrq:eqpwb}
                \State \Return \OK{} \label{pcrq:eqretOK}
            \EndIf
        \EndIf
        \State $\localHead{}\gets \Head{}$ \Comment{read \Head{}} \label{pcrq:headread}
        \If{$\localTail{}-\localHead{}\geq R$ \textbf{or} \Call{starving}{}}\label{pcrq:eqclosedchk}
            \State \Call{Test\&Set}{$\Tail{}.\var{cb}$} \label{pcrq:eqts}
            \State \recoverycode{\pwb{\Tail};} \recoverycode{\psync{}} \label{pcrq:closed-pwb-2}
            \State \recoverycode{$\var{closedFlag} \gets 1$}
            \State \Return \CLOSED{} \label{pcrq:eqclosedret}
        \EndIf
    \EndWhile
\EndFunction
\medskip% \Statex
%
%%% DEQUEUE FUNCTION %%%
\Function{Dequeue}{\crqV}
    \While{\True{}} \label{pcrq:dqouterloop}
        \State $\localHead\gets \Call{Fetch\&Increment}{\Head}$ \label{pcrq:dqfaa}
        \State $e\gets \Q[\localHead\bmod R]$ \label{pcrq:dqr1} \Comment{read item}
        \While{\True{}}
            \State $v\gets e.v$ \label{pcrq:dqr2} \Comment{read item's value}
            \State $( s,i) \gets ( e.s,e.\var{idx})$ \label{pcrq:dqr3} 
            \If{$i>\localHead{}$} \label{pcrq:dqichk}
                \textbf{goto} line \ref{pcrq:fix} \label{pcrq:enddqr2}
            \EndIf
            \If{$v\neq \bot$} \label{pcrq:dqemptychk}
                \If{$i == \localHead{}$} \label{pcrq:dqhchk}
                    \If{\Call{CAS2}{$\Q[\localHead\bmod R]$,$( s,\localHead,v)$,$( s,
                    \localHead{}+R,\bot)$}} \Comment{dequeue transition} \label{pcrq:dqtran}
                        \State \recoverycode{\pwb{\Head{}};} \recoverycode{\psync{}} \label{pcrq:dqpwbHead}
                        \State \Return $v$ \label{pcrq:dqret}
                    \EndIf
                \Else
                    \If{\Call{CAS2}{$\Q[\localHead\bmod R],( s,i,v) ,( 0,i,v)$}} 
                    \label{pcrq:unsafe} \Comment{unsafe transition}
                        \State \textbf{goto} line \ref{pcrq:fix} \label{pcrq:endunsafe}
                    \EndIf
                \EndIf
            \Else
                \If{\Call{CAS2}{$\Q[\localHead\bmod R],( s,i,\bot) ,( s,\localHead+R,
                \bot)$}} \Comment{empty transition} \label{pcrq:empty-1}
                    \State \textbf{goto} line \ref{pcrq:fix} \label{pcrq:endempty}
                \EndIf
            \EndIf
        \EndWhile
        \State $( \var{cb},\localTail{}) \gets$ \Tail \label{pcrq:fix}
        \If{$\localTail{}\leq \localHead{}+1$} \label{pcrq:empty}
            \State \recoverycode{\pwb{\Head};} \recoverycode{\psync{}} \label{pcrq:dqpwbHead2}
            \State \Call{FixState}{\crqV}
            \State \Return \EMPTY \label{pcrq:endfix}
        \EndIf
    \EndWhile
\EndFunction
\medskip
%
%%% FIX STATE %%%
\Function{FixState}{crq}
\While{True}
    \State $h\gets$ \Call{Fetch\&Add}{crq.head, 0}
    \State $t\gets$ \Call{Fetch\&Add}{crq.tail, 0}
    \If{$\text{crq.tail}\neq t$}
        \State \textbf{continue}
    \EndIf
    \If{$h\leq t$}
        \State \Return
    \EndIf
    \If{$\Call{CAS}{\text{crq.tail}, t, h}$}
        \State \Return
    \EndIf
\EndWhile
\EndFunction
\medskip
%\end{algorithmic}
%\end{multicols}
%\begin{multicols}{2}
%\begin{algorithmic}[1]
%\setcounter{ALG@line}{58}
%
%%% RECOVERY FUNCTION %%%
\recoverycode{
\Function{Recovery}{}
%\LComment{Parameters}
\State $R\colon$ size of circular array
%\Statex
%\LComment{Implementation}
\State $( \var{cb}, \localTail) \gets \Tail$ \label{pcrq:rec-tail-read}
\State $\Tail\gets ( \var{cb}, 0 )$
\For{$i\gets 0;\ i < R;\ i\texttt{++}$} \label{pcrq:rec-tail-loop}
    \If{$\Q[i].\var{val} \neq \bot$
	    \textbf{and} $\Tail < \Q[i].\var{idx} + 1$} \label{pcrq:rec-tail-occupiedchk}
	%        \LComment{occupied node and index is greater than current \Tail, hence update}
	        \State $\Tail\gets \Q[i].\var{idx} + 1$ \label{pcrq:rec-tail-set2}
    \ElsIf{$\Q[i].\var{val} == \bot$
    \textbf{and} $\Q[i].\var{idx} \geq R$} \label{pcrq:rec-tail-emptychk}
        \If{$\Tail < \Q[i].\var{idx} - R + 1$}
%            \LComment{empty node due to either a normal dequeue or an empty transition, and 
%            index $-R$ greater than current \Tail, hence update}
            \State $\Tail\gets \Q[i].\var{idx} - R + 1$ \label{pcrq:rec-tail-set1}
        \EndIf
    \EndIf
\EndFor
\If{$\Head>\Tail$} $\Tail\gets \Head$ \Comment{Empty queue} \label{pcrq:recemptycheck}
\Else \Comment{$\Head\leq \Tail$}
%    \LComment{Fix \Head\ to start from maximum index of unoccupied nodes $+1$}
    \State $\var{max} \gets \Head$ \label{pcrq:recinimax}
    \For{$i\gets \Head$;\ $i \bmod R \neq \Tail \bmod R$;\ $i\texttt{++}$} \label{pcrq:recmaxfor}
        \If{$\Q[i \bmod R].\var{val} == \bot$ \textbf{and}\\
        \hspace*{0.5em} $\Q[i \bmod R].\var{idx} - R > \var{max}$}
        \label{pcrq:recgtmax}
            \State $\var{max}\gets \Q[i \bmod R].\var{idx} - R + 1$
            \label{pcrq:recsetmax}
        \EndIf
    \EndFor
    \State $\Head \gets \var{max}$ \label{pcrq:rec-max-found}
%    \LComment{Fix \Head\ to start from minimum index of occupied nodes in $(\Head,\Tail]$}
    \State $\var{min} \gets \Tail$ \label{pcrq:rec-min-ini}
    \For{$i\gets \Head$;\ $i \bmod R \neq \Tail \bmod R$;\ $i\texttt{++}$}
        \If{$\Q[i \bmod R].\var{val} \neq \bot$
        \textbf{and} $\Q[i \bmod R].\var{idx} < \var{min}$
        \textbf{and} $\Q[i \bmod R].\var{idx} \geq \Head{}$} 
        \label{pcrq:recgteHead}
            \State $\var{min}\gets \Q[i \bmod R].\var{idx}$
        \EndIf
    \EndFor
    \If{$\var{min} < \Tail$} $\Head \gets \var{min}$ \label{pcrq:rec-min-found} \EndIf
\EndIf
%\LComment{Reset the rest of the array's positions}
\For{$i = \Head - 1;\ i \bmod R \neq \Tail \bmod R;\ i\texttt{--}$} \label{pcrq:resetloop}
    \State $\Q[i \bmod R] \gets ( 1, i+R, \bot)$ \label{pcrq:resetnodes}
\EndFor
%\LComment{Reset all safe flags to $1$}
\For{$i = 0;\ i < R;\ i\gets i + 1$} $\Q[i].s \gets 1$ \label{pcrq:resetsfloop1} \EndFor
\EndFunction        
}
\end{algorithmic}
\end{multicols}
\end{algorithm}


==> related.tex <==
\section{Related Work}
1 page.

